A measurement of Hubble's Constant using Fast Radio Bursts

We constrain the Hubble constant H$_0$ using Fast Radio Burst (FRB) observations from the Australian Square Kilometre Array Pathfinder (ASKAP) and Murriyang (Parkes) radio telescopes. We use the redshift-dispersion measure (`Macquart') relationship, accounting for the intrinsic luminosity function, cosmological gas distribution, population evolution, host galaxy contributions to the dispersion measure (DM$_{\rm host}$), and observational biases due to burst duration and telescope beamshape. Using an updated sample of 16 ASKAP FRBs detected by the Commensal Real-time ASKAP Fast Transients (CRAFT) Survey and localised to their host galaxies, and 60 unlocalised FRBs from Parkes and ASKAP, our best-fitting value of H$_0$ is calculated to be $73_{-8}^{+12}$ km s$^{-1}$ Mpc$^{-1}$. Uncertainties in FRB energetics and DM$_{\rm host}$ produce larger uncertainties in the inferred value of H$_0$ compared to previous FRB-based estimates. Using a prior on H$_0$ covering the 67--74 km s$^{-1}$ Mpc$^{-1}$ range, we estimate a median DM$_{\rm host} = 186_{-48}^{+59}$ km s$^{-1}$ Mpc$^{-1}$, exceeding previous estimates. We confirm that the FRB population evolves with redshift similarly to the star-formation rate. We use a Schechter luminosity function to constrain the maximum FRB energy to be $\log_{10} E_{\rm max}=41.26_{-0.22}^{+0.27}$ erg assuming a characteristic FRB emission bandwidth of 1 GHz at 1.3 GHz, and the cumulative luminosity index to be $\gamma=-0.95_{-0.15}^{+0.18}$. We demonstrate with a sample of 100 mock FRBs that H$_0$ can be measured with an uncertainty of $\pm 2.5$ km s$^{-1}$ Mpc$^{-1}$, demonstrating the potential for clarifying the Hubble tension with an upgraded ASKAP FRB search system. Last, we explore a range of sample and selection biases that affect FRB analyses.

==> Tables/orig_tab_MC.tex <==
\begin{table*}
\centering
\begin{minipage}{170mm} 
\caption{\changed{Monte Carlo FRBs generated for the (in development) CRACO system on ASKAP (see Section \ref{sec:craco_mc_results})}. \label{tab:MC}}
\begin{tabular}{cccc}
\hline 
Index & DM & \snr & $z$ 
\\ 
 & (\dmunits) 
\\ 
\hline 
0& 186.7& 15.9& 0.15\\ 
1& 1179.5& 26.0& 1.321\\ 
2& 438.5& 20.2& 0.062\\ 
3& 315.3& 17.9& 0.089\\ 
4& 833.1& 10.5& 0.949\\ 
5& 595.3& 32.8& 0.25\\ 
6& 313.4& 16.8& 0.37\\ 
7& 568.5& 13.1& 0.629\\ 
8& 143.5& 11.0& 0.026\\ 
9& 743.4& 12.6& 0.812\\ 
10& 941.9& 10.0& 0.755\\ 
11& 460.5& 10.7& 0.355\\ 
12& 1271.8& 12.1& 0.432\\ 
13& 1308.6& 15.7& 1.273\\ 
14& 567.9& 12.4& 0.608\\ 
15& 410.5& 84.7& 0.057\\ 
16& 391.1& 117.3& 0.251\\ 
17& 1287.8& 9.7& 1.592\\ 
18& 634.8& 15.9& 0.378\\ 
19& 383.0& 15.6& 0.176\\ 
20& 372.7& 16.2& 0.167\\ 
21& 237.3& 13.3& 0.041\\ 
22& 478.8& 27.0& 0.354\\ 
23& 835.0& 51.2& 0.735\\ 
24& 282.6& 10.6& 0.263\\ 
25& 151.4& 223.4& 0.046\\ 
26& 819.9& 13.1& 0.75\\ 
27& 162.3& 17.3& 0.138\\ 
28& 371.1& 25.0& 0.282\\ 
29& 357.4& 16.3& 0.262\\ 
30& 331.8& 40.2& 0.085\\ 
31& 557.5& 88.5& 0.289\\ 
32& 818.5& 9.8& 0.66\\ 
33& 1257.6& 22.4& 0.699\\ 
34& 1116.3& 11.6& 1.367\\ 
35& 2259.2& 12.3& 1.338\\ 
36& 307.9& 22.6& 0.243\\ 
37& 1311.1& 24.4& 1.712\\ 
38& 848.2& 11.6& 1.006\\ 
39& 1060.6& 10.6& 1.108\\ 
40& 785.5& 10.0& 0.164\\ 
41& 484.9& 11.7& 0.52\\ 
42& 481.2& 9.6& 0.424\\ 
43& 484.7& 14.9& 0.61\\ 
44& 260.6& 12.9& 0.054\\ 
45& 393.8& 12.7& 0.291\\ 
46& 273.7& 22.7& 0.182\\ 
47& 534.4& 21.0& 0.556\\ 
48& 703.6& 10.8& 0.195\\ 
49& 335.9& 18.5& 0.329\\
\hline 
\end{tabular}
\begin{tabular}{cccc}
\hline 
Index & DM & \snr & $z$ 
\\ 
 & (\dmunits) 
\\ 
\hline 
50& 898.1& 32.2& 0.718\\ 
51& 582.2& 13.8& 0.571\\ 
52& 636.2& 23.1& 0.441\\ 
53& 735.7& 27.7& 0.482\\ 
54& 1405.0& 11.4& 1.318\\ 
55& 1083.0& 19.3& 1.101\\ 
56& 709.4& 12.4& 0.58\\ 
57& 1794.1& 14.9& 1.849\\ 
58& 736.2& 11.0& 0.546\\ 
59& 808.6& 33.4& 0.472\\ 
60& 352.0& 16.0& 0.126\\ 
61& 447.5& 38.3& 0.543\\ 
62& 1346.2& 12.3& 1.567\\ 
63& 428.3& 12.3& 0.537\\ 
64& 421.8& 28.0& 0.018\\ 
65& 602.3& 16.3& 0.093\\ 
66& 1110.1& 94.0& 0.439\\ 
67& 303.5& 10.8& 0.137\\ 
68& 799.7& 18.8& 0.465\\ 
69& 309.6& 30.0& 0.159\\ 
70& 3446.6& 25.6& 0.08\\ 
71& 721.5& 25.8& 0.306\\ 
72& 296.3& 21.4& 0.134\\ 
73& 573.2& 19.6& 0.464\\ 
74& 184.5& 11.4& 0.063\\ 
75& 580.0& 15.6& 0.632\\ 
76& 754.0& 9.6& 0.103\\ 
77& 391.9& 11.2& 0.43\\ 
78& 282.0& 21.7& 0.073\\ 
79& 548.7& 25.8& 0.35\\ 
80& 449.7& 12.6& 0.019\\ 
81& 187.9& 40.8& 0.052\\ 
82& 522.1& 11.8& 0.353\\ 
83& 233.3& 85.5& 0.081\\ 
84& 923.9& 9.9& 0.961\\ 
85& 568.1& 15.9& 0.295\\ 
86& 1327.1& 18.6& 0.437\\ 
87& 901.0& 39.8& 0.744\\ 
88& 776.9& 14.5& 0.786\\ 
89& 359.8& 46.4& 0.372\\ 
90& 733.7& 18.7& 0.633\\ 
91& 685.6& 9.8& 0.765\\ 
92& 568.9& 14.8& 0.644\\ 
93& 398.7& 23.3& 0.239\\ 
94& 664.2& 15.8& 0.495\\ 
95& 326.6& 14.2& 0.251\\ 
96& 726.0& 23.7& 0.089\\ 
97& 342.1& 48.2& 0.029\\ 
98& 376.5& 47.9& 0.279\\ 
99& 271.9& 18.9& 0.237\\ 
\hline 
\end{tabular} 
\end{minipage} 
\end{table*} 


==> Tables/tab_results.tex <==
\begin{table}
\renewcommand{\arraystretch}{1.5}
    \centering
     \begin{tabular}{c|c c c c c}
     Parameter & Best Fit & 68\%  & 90\%  & 95\% & 99.7\% \\
     \hline
      \Hnot & 73.0 & $_{-8}^{+12}$ & $_{-12}^{+22}$ & $_{-13}^{+29}$ & $_{-17}^{+48}$  \\
     \lemax & 41.26 & $_{-0.22}^{+0.27}$ & $_{-0.33}^{+0.50}$ & $_{-0.38}^{+0.64}$ & $_{-0.51}^{+1.02}$  \\
     $\alpha$ & -1.00 & $^{+0.57}_{-0.59}$  & $^{+0.81}_{-0.87}$ & $^{+0.88}_{-0.96}$  & $^{+0.98}_{-1.00}$   \\
     $\gamma$ & -0.95   & $^{+0.18}_{-0.15}$ & $^{+0.30}_{-0.23}$ & $^{+0.36}_{-0.27}$ & $^{+0.45}_{-0.36}$   \\
     \sfrn & 1.13  & $_{-0.41}^{+0.49}$ & $_{-0.65}^{+0.77}$  & $_{-0.78}^{+0.89}$  & $_{-1.09}^{+1.19}$   \\
     \muhost & 2.27 & $_{-0.13}^{+0.12}$  & $_{-0.23}^{+0.20}$  & $_{-0.28}^{+0.25}$  & $_{-0.47}^{+0.33}$   \\
     \sigmahost & 0.55  & $_{-0.09}^{+0.11}$ & $_{-0.14}^{+0.21}$  & $_{-0.16}^{+0.28}$ & $_{-0.21}^{+0.51}$    \\
    \end{tabular}
    \caption{Best-fit parameter values and associated confidence intervals.}
    \label{tab:confidence_intervals}
\end{table}

%H0
%limits  0.00135 55.97597597597598 120.84084084084084
%limits  0.0228 59.729729729729726 101.6966966966967
%limits  0.05 61.45645645645646 95.31531531531532
%limits  0.15866 65.28528528528528 85.03003003003003


==> Unused/readme.tex <==
The six 'alpha.png' etc files are from our CRACO study, and didn't make it into the final manuscript

dm_by_snr was originally part of the appendix but is now removed - do not need this extra discussion

==> Unused/tab_MC_sub.tex <==
\begin{table}
\centering
\begin{minipage}{170mm} 
\caption{CRACO Monte Carlo\label{tab:MC}}
\begin{tabular}{cccc}
\hline 
Index & DM & \snr & $z$ 
\\ 
 & (\dmunits) 
\\ 
\hline 
0& 186.7& 15.9& 0.15\\ 
1& 1179.5& 26.0& 1.321\\ 
2& 438.5& 20.2& 0.062\\ 
3& 315.3& 17.9& 0.089\\ 
4& 833.1& 10.5& 0.949\\ 
5& 595.3& 32.8& 0.25\\ 
6& 313.4& 16.8& 0.37\\ 
7& 568.5& 13.1& 0.629\\ 
8& 143.5& 11.0& 0.026\\ 
9& 743.4& 12.6& 0.812\\ 
10& 941.9& 10.0& 0.755\\ 
11& 460.5& 10.7& 0.355\\ 
12& 1271.8& 12.1& 0.432\\ 
13& 1308.6& 15.7& 1.273\\ 
14& 567.9& 12.4& 0.608\\ 
15& 410.5& 84.7& 0.057\\ 
\hline 
\end{tabular} 
\end{minipage} 
\end{table} 


==> Unused/tab_frbs.tex <==
\begin{table*}
\centering
\begin{minipage}{170mm} 
\caption{Fast Radio Bursts Analyzed\label{tab:frbs}}
\begin{tabular}{cccccccc}
\hline 
Name & Survey & DM & $\nu$ & SNR & RA & Dec & $z$ \\
& & (pc cm$^{-3}$) & (MHz) & & (J2000) & (J2000) & 
\\ 
\hline 
20180924& CRAFT/ICS& 362.4& 1297.5& 21.1& 21:44:25.255& -40:54:00.1& 0.3214\\ 
20181112& CRAFT/ICS& 589.0& 1297.5& 19.3& 21:49:23.630& -52:58:15.39& 0.4755\\ 
20190102& CRAFT/ICS& 364.5& 1271.5& 14.0& 21:29:39.70836& -79:28:32.2845& 0.291\\ 
20190608& CRAFT/ICS& 339.5& 1271.5& 16.1& 22:16:04.7472s& -07:53:53.6& 0.1178\\ 
20190611.2& CRAFT/ICS& 322.2& 1271.5& 9.3& 21:22:58.372& -79:23:51.284& 0.378\\ 
20190711& CRAFT/ICS& 594.6& 1271.5& 23.8& 21:57:40.012& -80:21:28.18& 0.522\\ 
20190714& CRAFT/ICS& 504.7& 1271.5& 10.7& 12:15:55.081& -13:01:14.36& 0.209\\ 
20191228& CRAFT/ICS& 297.5& 1271.5& 22.9& 22:57:43.269& -29:35:37.85& 0.243\\ 
20210407& CRAFT/ICS& 1785.3& 1271.5& 19.1& 05:14:36.202& 27:03:30.24& -1.0\\ 
\hline 
\end{tabular} 
\end{minipage} 
\end{table*} 


==> Unused/tab_model_params_CJ.tex <==
\begin{table*}
\centering
\begin{minipage}{170mm} 
\caption{Fiducial Set of Model Parameters. Parametrs labelled with a `^*' are re-fit as part of this work.\label{tab:param}}
\begin{tabular}{cccl}
\hline 
Parameter & Fiducial Value & Unit & Description 
\\ 
\hline 
$\mu_{w}$& 1.70267& ms & $log_{10}$ mean of intrinsic width distribution in ms\\ 
$\sigma_{w}$& 0.899148 & ms& $log_{10}$ sigma of intrinsic width distribution in ms\\ 
$\log \mu_s$ & 0.7 & ms &  Mean of log-scattering distribution at 600\,Mhz \\
$\log \sigma_s$ & 1.72 & ms & Standard deviation of log-scattering distribution at 600\,MHz \\
%$w_{m min}$& 0.5& & Starting fraction of intrinsic width for histogramming\\ 
\dmcosmic & & \dmunits & Cosmological DM contribution. \\
\dmism & NE2001 & \dmunits & DM for the Milky Way Interstellar Medium \\
\dmhalo & 50& \dmunits & DM for the Galactic halo\\ 
$\mu_{\rm host}$ $^*$& 2.18& & $log_{10}$ mean of DM host contribution in pc cm$^{-3}$\\ 
$\sigma_{\rm host}$ $^*$& 0.48& & $log_{10}$ sigma of DM host contribution in pc cm$^{-3}$\\
\sfrn$^*$ & 0.73& & scaling of FRB rate density with star-formation rate\\ 
\Hnot$^*$& 67.66& \dmunits & Hubble's constant\\ 
$\Omega_{\Lambda}$& 0.68885& & dark energy / cosmological constant (in current epoch)\\ 
\omegam & 0.30966& & matter density in current epoch\\ 
\omegab & 0.04897& & baryon density in current epoch\\ 
\omegabhh & 0.02242& & baryon density weighted by $h_{100}^2$\\ 
$F$& 0.32& & F parameter in DM$_{\rm cosmic}$ PDF for the Cosmic web\\ 
\fdzo & 0.844 & & fraction of baryons that are diffuse and ionized at $z=0$. \\
\lemin$^*$& 30& erg& $log_{10}$ of minimum FRB energy \\ 
\lemax$^*$& 41.4& erg& $log_{10}$ of maximum FRB energy\\ 
$\alpha$$^*$& -0.65& & power-law index of frequency dependent FRB rate, $R \sim \nu^alpha$\\ 
$\gamma$$^*$& -1.01& & slope of luminosity distribution function\\ 
\hline 
\end{tabular} 
\end{minipage} 
\end{table*} 

